Redefining Affordance via Computational Rationality

Affordances, a foundational concept in human-computer interaction and design, have traditionally been explained by direct-perception theories, which assume that individuals perceive action possibilities directly from the environment. However, these theories fall short of explaining how affordances are perceived, learned, refined, or misperceived, and how users choose between multiple affordances in dynamic contexts. This paper introduces a novel affordance theory grounded in Computational Rationality, positing that humans construct internal representations of the world based on bounded sensory inputs. Within these internal models, affordances are inferred through two core mechanisms: feature recognition and hypothetical motion trajectories. Our theory redefines affordance perception as a decision-making process, driven by two components: confidence (the perceived likelihood of successfully executing an action) and predicted utility (the expected value of the outcome). By balancing these factors, individuals make informed decisions about which actions to take. Our theory frames affordances perception as dynamic, continuously learned, and refined through reinforcement and feedback. We validate the theory via thought experiments and demonstrate its applicability across diverse types of affordances (e.g., physical, digital, social). Beyond clarifying and generalizing the understanding of affordances across contexts, our theory serves as a foundation for improving design communication and guiding the development of more adaptive and intuitive systems that evolve with user capabilities.

==> tex/5.application.tex <==
\section{Novel Capabilities Enabled by Our Theory}

Our CR-based affordance theory introduces several new capabilities that go beyond traditional affordance theories. While traditional views focus on affordances as properties directly perceived in the external environment, our theory emphasizes the construction of affordance perception within an internal environment and the role of learning and decision-making in shaping affordance detection. Below, we highlight key novel capabilities enabled by our theory that traditional models cannot fully address.

\subsection{Affordance Perception as a Constructive Process}

One of the fundamental advancements of our theory is the shift from perceiving affordances directly from the external environment to understanding affordance perception as a \textit{constructive, internally-driven process}. According to our model, users infer affordances based on their internal representation of the environment, which is constructed from limited sensory input and past experience.

Traditional affordance models assume a direct alignment between environmental affordances and their perception. However, this approach falls short in \textit{novel} or \textit{ambiguous environments}, where sensory data may be incomplete or unfamiliar. Our theory, by emphasizing internal representations, better explains how users adapt to new environments or situations—such as digital interfaces—where affordances may not be obvious or physically embedded.

\subsection{Incorporation of Decision-Making Through Confidence and Predicted Utility}

A novel contribution of our theory is the introduction of \textit{confidence} (the perceived likelihood of successfully performing an action) and \textit{predicted utility} (the expected value of the outcome). These two factors are key to understanding how users evaluate affordances and make decisions when presented with multiple action possibilities.

Traditional affordance models describe whether an affordance exists but don’t explain how users make choices between affordances. Our theory goes further by integrating decision theory, enabling designers to model how users weigh \textit{risk}, \textit{reward}, and \textit{uncertainty} when choosing actions. This is particularly important in \textit{complex systems}, where users must choose between several affordances, each with varying levels of success and utility.

\subsection{Learning and Refinement of Affordances Over Time}

Our theory recognizes that affordances are \textit{learned and refined} through \textit{reinforcement learning}. Rather than viewing affordances as static features of the environment, we argue that users continuously update their internal models based on the feedback they receive from interacting with the world.

Traditional affordance theories, including Gibson’s, do not explain how affordances evolve through interaction. By modeling how users refine their understanding of affordances over time—through trial and error, success, and failure—our theory provides a \textit{dynamic view} of affordance perception. This capability allows designers to create interfaces or systems that facilitate affordance learning through clear feedback and interaction cues.

\subsection{Inferring Others’ Affordances}

A significant novel aspect of our theory is its ability to explain how we infer the affordances of \textit{others}. In social and collaborative contexts, users often need to infer what actions others can perform in an environment. Our theory explains this by extending the same mechanisms used for perceiving one’s own affordances to others. Through \textit{hypothetical motion trajectories} and \textit{internal models}, individuals can simulate the potential actions of others, allowing them to infer what others can do even without directly observing the action.

Traditional affordance theories, such as Gibson’s, focus on the direct perception of affordances relative to the observer, but they do not fully address how we infer others' affordances. By incorporating \textit{internal simulations}, our theory enables individuals to understand others' action possibilities, making it applicable in social contexts, collaborative environments, and human-robot interaction.

\subsection{Affordances in Digital and Virtual Environments}

One contribution of our theory is its applicability to \textit{digital and virtual environments}. In these spaces, affordances are not tied to physical objects but instead emerge through interaction design. Our theory explains how users perceive and learn affordances by constructing internal representations based on \textit{digital feedback} and prior experiences with interface elements, allowing designers to better shape user interactions in \textit{non-physical environments}.

Gibson’s theory, developed in the context of physical environments, has limitations when applied to \textit{virtual spaces}. By contrast, our theory excels in explaining how users perceive affordances in \textit{digital interfaces}, making it highly relevant for \textit{HCI}, \textit{UX design}, and \textit{AI-based interaction systems}.

\subsection{Conclusion}

In summary, our affordance theory offers several \textit{new capabilities} that traditional models cannot fully address:
\begin{itemize}
    \item It emphasizes \textit{affordance perception as a constructive process}, occurring within an internal model.
    \item It incorporates \textit{decision-making}, allowing users to weigh \textit{confidence} and \textit{predicted utility} when choosing between affordances.
    \item It models \textit{learning and refinement} through \textit{reinforcement}, allowing for a more dynamic understanding of affordance perception.
    \item It explains how users infer \textit{others' affordances} through internal simulations and hypothetical trajectories.
    \item It is particularly powerful in explaining affordances in \textit{digital and virtual environments}, providing a framework for designing \textit{non-physical systems}.
\end{itemize}

By addressing these gaps, our theory enhances both the theoretical understanding of affordance perception and offers practical insights for designing user-centered systems in both physical and digital environments.

